Example-Based Vulnerability Detection and Repair in Java Code

The Java libraries JCA and JSSE offer cryptographic APIs to facilitate secure coding. When developers misuse some of the APIs, their code becomes vulnerable to cyber-attacks. To eliminate such vulnerabilities, people built tools to detect security-API misuses via pattern matching. However, most tools do not (1) fix misuses or (2) allow users to extend tools' pattern sets. To overcome both limitations, we created Seader-an example-based approach to detect and repair security-API misuses. Given an exemplar <insecure, secure>code pair, Seader compares the snippets to infer any API-misuse template and corresponding fixing edit. Based on the inferred info, given a program, Seader performs inter-procedural static analysis to search for security-API misuses and to propose customized fixes. For evaluation, we applied Seader to 28 <insecure, secure> codepairs; Seader successfully inferred 21 unique API-misuse templates and related fixes. With these <vulnerability, fix> patterns, we applied SEADER to a program benchmark that has 86 known vulnerabilities. Seader detected vulnerabilities with 95% precision, 72% recall, and82% F-score. We also applied Seader to 100 open-source projects and manually checked 77 suggested repairs; 76 of the repairs were correct. Seader can help developers correctly use security APIs.

==> Result/EvaluationDesign.tex <==
% question, related work, ruleset, extendsion. addtional rule. extendsion. example. flexible.  

\section{Evaluation}
This section describes the training data set and the performance of our tool on the test data set and the pattern we generated, and then we present our research questions (RQs) and its results. Finally, we discuss the limitation of the tools in the current implementation status. 

\subsection{Data Set}
\textbf{Training dataset} We use the data set crawled from StackOverflow, which related to cryptography API usage~\cite{chen2019reliable}; this dataset includes 785 secure answer posts and 644 insecure answer posts. We further 1) paired the insecurity code examples with the corresponding security codes; 2) pruned unrelated code to make each code example only includes one of the vulnerability; 3) constructed the code snippets to the compilable program and manually fixed the vulnerability code snippet if there is no matched security code snippet in the dataset. Since there are a lot of code snippets reflect the same API misuse case, we also removed the duplicated case. Overall, we have a training dataset which contains 72 pair of codes. Since the options for writing the insecure codes and secure codes are limited, the number of the training dataset is unnecessary to be large.

% \begin{listing*}
%     \begin{minted}[mathescape,
%                   linenos,
%                   breaklines,
%                   numbersep=5pt,
%                   gobble=0,
%                   fontsize=\small,
%                   frame=lines,
%                   framesep=2mm]{java}
% public class EcbInSymmCryptoABICase1 {
%     public void go(String crypto) throws NoSuchPaddingException, NoSuchAlgorithmException, InvalidKeyException {
%         KeyGenerator keyGen = KeyGenerator.getInstance("AES");
%         SecretKey key = keyGen.generateKey();
%         Cipher cipher = Cipher.getInstance(crypto);
%         cipher.init(Cipher.ENCRYPT_MODE, key);
%     }

%     public static void main (String [] args) throws NoSuchPaddingException, NoSuchAlgorithmException, InvalidKeyException {
%         EcbInSymmCryptoABICase1 bc = new EcbInSymmCryptoABICase1();
%         String crypto = "AES/ECB/PKCS5Padding";
%         bc.go(crypto);
%     }
% }
%     \end{minted}
%     \caption{The Code Causing Wrong Parameter Retrieval}
%     \label{exp:wrong}
% \end{listing*}


==> Result/EvaluationPattern.tex <==
\subsection{Pattern Generation}
Before we compare to state-of-the-art, we first use our train dataset to generate the template for detection. For each pair of the code, this tool generates the API misuse pattern by analyzing the code difference. It extracts the binding information for invoked API, records the API name with incorrect usage format, and the fixed operation. This tool generates 13 patterns from the training dataset. We categorized these pattern into Four different part:  

\textbf{Parameter pattern:} This pattern related to the encryption algorithm misuse within a method invocation. The incorrect and correct usage of algorithms could be enumerated and the fixed method is updating the algorithm with the correct one.

\textbf{Number pattern:} This pattern related to incorrect usage of number value range such as key size.  Compared with parameter pattern, this pattern should reflect the incorrect value range information, so when fixing such vulnerabilities, we need to compare the value range information and picked a security value.  

\textbf{Name Pattern:} This pattern related to the API name replacement. 

\textbf{Composite pattern:} This pattern includes a block of the code statements replaced with another block of the statements. For example, a static declared password should be replaced with a randomly generated password. 

% \todo[inline]{one rule, one categories. multi-line, vulnerability, comparision with other tools}

The generated pattern is shown in Table~\ref{tab:Pattern}. When checking the parameter and number, SAFI will also generate the index of arguments need to be checked. 

\begin{table}[hbtp]
    \centering
    \begin{tabular}{c|c}
        Pattern Type & Inspection Function\\
        \hline
        \multirow{8}{*}{Parameter} & Cipher.getInstance\#0 \\& MessageDigest.getInstance\#0 \\ & SSLContext.getInstance\#0 \\ & SecretKeySpec.<init>\#0 \\ & SecureRandom.setSeed\#0 \\ & IvParameterSpec.<init>\#0 \\ & PBEKeySpec.<init>\#0 \\ & PBEKeySpec.<init>\#1 \\
        \hline
        \multirow{2}{*}{Number} & KeyPairGenerator.initialize \\ & PBEKeySpec.<init>\#2 \\
        \hline
        Name & Random.<init> \\
        \hline
        \multirow{2}{*}{Composite Pattern} & Trust Manager \\ & HostnameVerifier \\
        \hline
    \end{tabular}
    \caption{Pattern Generation}
    \label{tab:Pattern}
\end{table}




==> Result/EvaluationRQ1.tex <==
%   1. comparsion how tool work compare state art, ,comparesion dataset,performace. time performace. include the time. based on 13 project. precision, recall. time, work. comparsion. introduce. 
\subsection{RQ1: How does the detection of SAFI compare to the state-of-the-art?}

We evaluate our tool and the state-of-the-art in the following dimensions:
\begin{itemize}
    \item Running Time: the execution time of tool to generate the result.
    \item Precision: the correctness of the result.
    \item Recall: \textcolor{red}{123}
    \item Configuration: How easy to add a new pattern.
\end{itemize}

To verify the correctness of detection, we choose CryptoAPI \footnote{\url{https://github.com/CryptoGuardOSS/cryptoapi-bench/tree/master/src/main/java/org/cryptoapi/bench}}, which includes 197 programs that covers 14 kinds of API misuse and 13 jar files which are from 100 open-source projects. The experiment result is shown at Table~\ref{tab:cryptoBench}, ~\ref{tab:Apache Running Time} and~\ref{tab:Apache Result}. 

The CryptoAPI is for testing the coverage of SAFI generated pattern template. In CryptoBench, it contains various methods of calling crypto API such as inter-procedural and intra-procedural call. It helps to examine if the detection tool can handle the common code usage in practical. As shown in Table~\ref{tab:cryptoBench}, we pass all 14 kinds of API misuses. Meanwhile, we manually review all the given fix. It all fits the original code context and can be compiled. 

Table~\ref{tab:Apache Running Time} and Table~\ref{tab:Apache Result} is for comparing the accuracy and the running time between SAFI and CryptoGuard against the practical projects.
For human inspection, we ask a student who has experience in security API and provides him a checklist. In general, SAFI can generate the result closer to human inspection and runs faster than the CryptoGuard. Note that human inspection might miss some cases, and it cannot be treated as ground truth. From Table~\ref{tab:Apache Result}, we conclude that 1) SAFI can find out more cases than humans; 2) SAFI can guide engineers where to change the code while CryptoGuard only prints wrong pattern for some cases; 3) SAFI and CryptoGuard have very close cases number in some cases. As for running time comparison, SAFI is faster than CryptoGuard except for one case \emph{flume-file-channel-1.9.0.jar}. The reason is that the slowest part of our process is to build the callgraph and the backward slicing. We use the Wala built-in functions. Although we have optimized the speed of building the callgraph and prune the callgraph, it is still slower than the CryptoGuard. Moreover, due to the callgraph generation, in some cases, the callgraph is not well reflected in the original code architecture. However, the other parts run fast. Based on our experiment, the actual security-related data-flow analysis takes less than two seconds among these 13 projects. In our future work, we will improve the callgraph and implement the security-related slicing to increase the speed further so that SAFI can give the suggestion in real-time. 



\begin{table*}[h]
    \centering
    \begin{tabular}{c|c|c|c|c}
        Category & Total Case\# & Correct Case \#  & SAFI Detected \# & SAFI Gave Fix \# \\
        \hline
        brokencrypto & 36 & 1 & 35 & 35\\
        \hline
        brokenhash & 28 & 1 &27 & 27\\
        \hline
        dummycertvalidation & 3 & 0 & 3 & 1 \\
        \hline
        dummyhostnameverifier & 4& 1 &3 &3\\
        \hline
        ecbcrypto & 8 & 1 &7 &5\\
        \hline
        http &9 &2 &9 &9\\
        \hline
        impropersslsocketfactory &4 &0 &4 &4\\
        \hline
        insecureasymmetriccrypto & 6 &1 &5 &3\\
        \hline
        pbeiteration &9 &1 &8 &8\\
        \hline
        predictablecryptographickey &10 &1 &9 &9\\
        \hline
        predictablepbepassword &11 &1 &10 &10\\
        \hline
        predictableSeeds & 17 &1 &16 &16\\
        \hline
        staticinitializationvector & 10 &1 &9 &9\\
        \hline
        staticsalts &9 &1 &8 &8\\
        \hline
        untrustedprng &2 &1 & 1 & 1\\
    \end{tabular}
    \caption{CryptoBench Result}
    \label{tab:cryptoBench}
\end{table*}

\begin{table*}[hbtp]
    \centering
    \begin{tabular}{c|c|c|c}
        Filename &  SAFI Running Time (s) & CryptoGuard Runtime(s) & File Size (KB)\\
        \hline
        apacheds-kerberos-codec-2.0.0.AM25.jar & 5.34 & 8.85 & 672\\
        \hline
        artemis-commons-2.11.0.jar & 4.58 & 6.31 & 360\\
        \hline
        deltaspike-core-impl-1.9.2.jar & 2.65 & 3.61 & 206\\
        \hline
        flume-file-channel-1.9.0.jar& 142.91 & 5.5 & 294\\
        \hline
        hadoop-hdfs-3.2.1.jar & 15.78 & 70.68 & 5820\\
        \hline
        jclouds-core-2.2.0.jar & 5.87 & 8.92 & 906\\
        \hline
        %shindig-common-3.0.0-beta4.jar & 3.51 & 4.12 & 311 \\
        % \hline
        shiro-crypto-cipher-1.5.0.jar & 2.02 & 1.85 & 24\\
        \hline
        wagon-provider-api-3.3.4.jar & 2.10 & 1.95 & 55\\
        \hline
        wss4j-ws-security-common-2.2.4.jar & 4.24 & 7.74 & 330\\
        \hline
        wss4j-ws-security-stax-2.2.4.jar & 2.25 & 6.67 & 400\\
        \hline
    \end{tabular}
    \caption{10 Apache Project Running Time Comparison}
    \label{tab:Apache Running Time}
\end{table*}


% corrected the table not include different rule. change the domian knowlwdge.  F1 score report  % crpto match with our rule. 

\begin{table*}[hbtp]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
        Filename &  \makecell{SAFI\\Found\\Cases (s)} & \makecell{CryptoGuard\\Found\\Cases} & \makecell{Human\\Inspection\\Cases} & \makecell{Precision \\ SAFI/Cryptoguard} & \makecell{Recall \\SAFI/CryptoGuard} & \makecell{F1 score \\ SAFI/Cryptoguard} \\
        \hline
        apacheds-kerberos-codec-2.0.0.AM25.jar & 21 & 5 & 10 & 1/1 & 1/0.5 & 1/0.67\\
        \hline
        artemis-commons-2.11.0.jar & 6 & 6 & 3 & 1/1 & 1/1 & 1/1\\
        \hline
        deltaspike-core-impl-1.9.2.jar & 1 & 1 & 1& 1/1 & 1/1 & 1/1\\
        \hline
        flume-file-channel-1.9.0.jar & 2 & 2 & 1 & 1/1 & 1/1 & 1/1\\
        \hline
        hadoop-hdfs-3.2.1.jar & 5 & 5 & 5 & 1/1 & 1/1 & 1/1\\
        \hline
        jclouds-core-2.2.0.jar & 6 & 5 & 2 & 1/1 & 1/1 & 1/1\\
        % \hline
        % shindig-common-3.0.0-beta4.jar & 2 & 3 & 2 & 1/1 & 0\\
        \hline
        shiro-crypto-cipher-1.5.0.jar & 2 & 1 & 0 & N/A & N/A & N/A\\
        \hline
        wagon-provider-api-3.3.4.jar & 1 & 1 & 0 &  N/A& N/A & N/A\\  
        \hline
        wss4j-ws-security-common-2.2.4.jar & 5 & 4 & 5 & 1/1 & 1/0.8 & 1/0.89\\
        \hline
        wss4j-ws-security-stax-2.2.4.jar &5 & 1 & 5 & 1/1 & 1/0.2 & 1/0.33\\
        \hline
    \end{tabular}}
    \caption{10 Apache Project Result Comparison}
    \label{tab:Apache Result}
\end{table*}

In summary, SAFI can generate the pattern and detect the common vulnerable cases at a speed that not slower than state-of-the-art. 

==> Result/EvaluationRQ2.tex <==
%  2. effective of the tool, real work project. 100 projects. 
\subsection{RQ2: How does SAFI perform on 100 Apache projects?}

To further study the performance and invulnerability against the real project, from Github, we download the top 100 project source codes that satisfy the following criteria:
\begin{itemize}
    \item It must be the Apache project.
    \item It has the crypto API calls.
\end{itemize}

% no experinece 
% professional check

We compiled the top 100 Apache projects sorted by stars. After compilation, the total number of jar files is 3578 since it contains the dependencies of projects. We use SAFI to check all these jar files, and the result is shown in Table~\ref{tab:100 projects}.

% {'Rule Cipher getInstance': 23,
%  'Rule IvParameterSpec <init>': 9,
%  'Rule KeyPairGenerator initialize': 0,
%  'Rule KeyStore load': 31,
%  'Rule MessageDigest getInstance': 116,
%  'Rule PBEKeySpec <init>': 9,
%  'Rule PBEParameterSpec <init>': 8,
%  'Rule Random <init>': 420,
%  'Rule SecretKeySpec <init>': 25,
%  'Rule SecureRandom setSeed': 0}

% show that in some case, the api is used in vulnerable but left in purpose or not for the security purpose

From Table~\ref{tab:100 projects}, SAFI found a lot of security issues in the Apache project. However, when we check the occurrence of the insecure code snippets, we find:
\begin{itemize}
    \item \textbf{A lot of insecure code is written in the unit test code.} For the simplicity of writing the unit test code, engineers will not focus if the code is secure. Since the testing code will not run in the production environment, and if it is insecure, it will not have the security issue. When we study the RQ3, we have manually filtered out all this testing code when we push the change.
    \item \textbf{TrustAllManager is common on the project.} In some scenarios, engineers have to trust all incoming connections. Hence they wrote a specific class named \emph{TrustAllManager}. In this case, SAFI will warn the user that this is not secure, but further actions need to be done by engineers, such as leave a comment to warn other engineers that this class is not secure.
    \item \textbf{Insecure crypto APIs are used for other purposes.} Generally, engineers need to verify the file integrity. They will use \emph{MessageDigest.getInstance(``MD5")} or ``SHA-1" in the code. Under this circumstance, the code will not have any security concern, although MD5 and SHA-1 are vulnerable to the collision attack. But if engineers use SHA-1 or MD5 to encrypt the password, it will be dangerous since the length of a password is much less than the file size typically.  
\end{itemize}

For the second and the third findings, SAFI cannot handle the scenario correctly because SAFI can only examine the code by its type and name. It cannot read the purpose of engineers to write the code. Hence, the result might have a lot of noise for the users. In the future, we will let SAFI more intelligent in catching the hidden security problem.  

==> Result/EvaluationRQ3.tex <==
%  3. evaluation fix patch, accpted, mannuly detected
\subsection{RQ3: How does the fix patch work in practical projects?}

To find out if SAFI is helpful, we submit 65 pull requests using SAFI suggestion to   Apache projects. We notice that in the unit test, some programs intentionally leave a "TrustAll" function that accepts all SSL connections without any certification. We have filtered out all these cases when pushing the merge requests. The result is shown at Table~\ref{tab:PR}:

% feedback mistual postive netural. pass the unit test. response, pass 
% mainly report  maintain project  
% follow up question. , user student statiscti. accept. positive quto the response.  

\begin{table}[hbtp]
    \centering
    \begin{tabular}{c|c}
        Status &  Total \# \\  
        \hline
        Merge & 3 \\
        \hline
        Positive Feedback (exclude merge) & 1 \\
        \hline
        Unit Test Passed & 14 \\
        \hline
        Negative feedback & 7 \\
        \hline
        No Feedback (without archived project) & 12 \\
        \hline
        Unit Test Failed & 12 \\
        \hline
        Others & 10 \\
        \hline
        TOTAL & 60
    \end{tabular}
    \caption{Vulnerability Detection}
    \label{tab:PR}
\end{table}

\begin{table*}[hbtp]
    \centering
    \begin{tabular}{c|c|c|c}
        Apache Project Name & Stars & Merge Link & Comments \\  
        \hline
        apache/pulsar & 5.4k & https://github.com/apache/pulsar/pull/6447 &  \\
        \hline
        apache/beam & 3.8k & https://github.com/apache/beam/pull/11008 & Merged by \#10055 \\
        \hline
        apache/servicecomb-java-chassis & 1.6k & https://github.com/apache/servicecomb-java-chassis/pull/1604 & \\
        \hline
    \end{tabular}
    \caption{Apache Merge Project}
    \label{tab:Merge}
\end{table*}


Note that Apache projects have more strict about accepting the merge request outside the core developer. Our fix suggestions are been merged by three high stars (5.4k, 3.8k and 1.6k) Apache projects. 

For the positive side, three project owners have merged the code. For the high stars projects, the project owner quickly replied our request and merge the request. And for eight projects, we pass the unit tests. 

For the negative feedback, some developers leave responses that for speed consideration, they won't change the current encryption algorithm. Meanwhile, they have also implemented some other codes based on a specific algorithm. If the current encryption algorithm changes, they need to make more consequence change, which might be risky for them. A few developers are not happy with our commit message since we did not elaborate on the reason why we change.  

For the unit test failed, we manually inspect the error message generated from the Continuous Integration(CI). It can be broken down in the following reason:
\begin{enumerate}
    \item CI did not allow external push. 
    \item CI machine is down.
    \item The java code formatting is wrong.
\end{enumerate}

Like others, some projects had archived in Github, while some projects did not accept merges on Github, etc.

In summary, SAFI can help the engineer to detect the insecure code snippets. In some cases, it will fail to tell if the crypto API is used for security purposes. 





==> Result/limitation.tex <==
\section{Threat To Validity}

In this section, we discuss the threats to validity. There are a few limitations to our tools: 
\begin{enumerate}
    \item \textbf{Focus on the Java application only.} SAFI can only detect the security-related API on Java application. For Android API, it has some different crypto API than Java. Besides, for the misuse in Javascript, SAFI cannot detect it. To detecting the crypto API misuse in the Android application, users can add the template to the JSON file and specify the entry point of the application. As Javascript, SAFI needs to make some changes to handle the different IR in javascript. 
    \item \textbf{Generating the callgraph and slicing can be slow.} As we mentioned before, based on our experiment, Wala built-in callgraph and the built-in static slicing function can be slow since the callgraph can be complicated. Besides, the static slicing algorithm will give an approximate result that the result might not be accurate in some cases. In the future, we will implement a callgraph and slicing algorithm that only focuses on the security-related code to shrink the size of the callgraph.
    \item \textbf{The fix suggestion is not taken consideration of the purpose of the code.} As we run our tool on the practical projects, we found that the vulnerable code is in a) the unit test code; b) left in purpose. For instance, the engineer will leave the code to trust all connections in SSL in the unit test. And the engineer will use the ``SHA-1" or "MD5" for the file validation. Although it is not a security-related code, they use the crypto API. For SAFI, it cannot tell if the engineer uses the crypto API for security purposes. For solving the report in the unit test, engineers can filter the result generated by SAFI to get rid of the testing code. For the second case, it needs to manually decide if the suggested fix is suitable for the current scenarios. 
    
\end{enumerate}
    


